Strong Model Collapse

Within the scaling laws paradigm, which underpins the training of large neural networks like ChatGPT and Llama, we consider a supervised regression setting and establish the existance of a strong form of the model collapse phenomenon, a critical performance degradation due to synthetic data in the training corpus. Our results show that even the smallest fraction of synthetic data (e.g., as little as 1\% of the total training dataset) can still lead to model collapse: larger and larger training sets do not enhance performance. We further investigate whether increasing model size, an approach aligned with current trends in training large language models, exacerbates or mitigates model collapse. In a simplified regime where neural networks are approximated via random projections of tunable size, we both theoretically and empirically show that larger models can amplify model collapse. Interestingly, our theory also indicates that, beyond the interpolation threshold (which can be extremely high for very large datasets), larger models may mitigate the collapse, although they do not entirely prevent it. Our theoretical findings are empirically verified through experiments on language models and feed-forward neural networks for images.

==> mnist-results.tex <==
\subsection{Experimental results for Neural Networks on MNIST}
\label{sec:mnist}
\begin{wrapfigure}{r}{0.43\textwidth}
    \centering
    \vspace{-.5cm}
    \includegraphics[width=1\linewidth]{ICLR 2025 Template/figs/nn_diff_width.pdf}
    \vspace{-.5cm}
    \caption{\small{{\bf Fully trained two-layer network on MNIST data. } Impact of model size (hidden dimension, aka network width) on model collapse. Here, the model is trained solely on synthetic data (i.e $p_2 \to 1$).}}
    \label{fig:nn_model_width}
 \vspace{-.5cm}
\end{wrapfigure}
\textbf{Setup.} For two-layer neural networks, we consider two scenarios: (1) learning with a random projection  model as in Section \ref{sec:nn_theory}, where the first layer of the network is fixed randomly, and only the second layer is trained, and (2) learning with a fully trainable neural network.
The first setting directly corresponds to our theoretical results from Section \ref{sec:nn_theory}, but with ReLU activation functions. In the case of fully trained neural networks in the second setting, our theory does not apply directly. However, we hypothesize that the general trends observed in our asymptotic theory will still hold: (1) there will be a significant model collapse, which only diminishes as the %mixing coefficient of the synthetic data, $\alpha$ ,
fraction of synthetic data approaches $0$; (2) larger models will exhibit a more severe model collapse.


To align with the theoretical setting, we employ a (multivariate) regression approach where labels are converted to one-hot vectors and the model is trained using mean squared error. The synthetic labels were generated by another two-layer network, with Gaussian label noise (standard deviation of 0.1) added. A validation set is used to select the best checkpoint, and evaluation is conducted on the test set using the clean labels. Further details of the training % process
are provided in Appendix \ref{sec:app-two-layer}.

\begin{figure}[tb]
    \centering
    \vspace{-.3cm}
    \includegraphics[width=.9\linewidth]{ICLR 2025 Template/figs/mixing_nn.pdf}
    \vspace{-.3cm}
    \caption{\small{\textbf{Model collapse as a function of the  proportion of synthetic data.} We use the MNIST dataset with regression loss. Error bars correspond to 5 runs. \textbf{Left}, Random feature model with hidden dimension 100,000. \textbf{Right}, Two-layer neural network of width (i.e hidden dim.) $m=2000$. }}
    \vspace{-.5cm}
    \label{fig:mnist_mix_ratios}
\end{figure}


\textbf{Results.} Figure \ref{fig:mnist_mix_ratios} presents the results for both random feature models (left) and fully trained neural networks (right). In these experiments, we mixed synthetic and original data in the training set with varying coefficients, $p_1$. As the proportion of synthetic data, $p_2$, increases, the scaling laws slow down and eventually plateau. We observe a strong model collapse: only when $p_2$ approaches 0 does the collapse subside. The results are consistent across both cases, validating our theoretical predictions and demonstrating the applicability of our insights to more complex scenarios.


We also investigated how model size, specifically the hidden dimension of fully trained neural networks, affects model collapse. As shown in Figure \ref{fig:nn_model_width}, models with varying hidden dimensions were trained exclusively on the synthetic dataset with $p_2=1$. For training sets ranging from 10,000 to 50,000 samples, our results indicate that larger models are more susceptible to model collapse under the same validation and evaluation protocols. Notably, all these models remain in the interpolation regime, aligning with our theoretical predictions.
